Social Links vs. Language Barriers: Decoding the Global Spread of Streaming Content

The development of the internet has allowed for the global distribution of content, redefining media communication and property structures through various streaming platforms. Previous studies successfully clarified the factors contributing to trends in each streaming service, yet the similarities and differences between platforms are commonly unexplored; moreover, the influence of social connections and cultural similarity is usually overlooked. We hereby examine the social aspects of three significant streaming services--Netflix, Spotify, and YouTube--with an emphasis on the dissemination of content across countries. Using two-year-long trending chart datasets, we find that streaming content can be divided into two types: video-oriented (Netflix) and audio-oriented (Spotify). This characteristic is differentiated by accounting for the significance of social connectedness and linguistic similarity: audio-oriented content travels via social links, but video-oriented content tends to spread throughout linguistically akin countries. Interestingly, user-generated contents, YouTube, exhibits a dual characteristic by integrating both visual and auditory characteristics, indicating the platform is evolving into unique medium rather than simply residing a midpoint between video and audio media.

==> distribution_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table}[]
\begin{tabular}{lllllllll}
Platform & \multicolumn{2}{l}{YouTube} & \multicolumn{2}{l}{Spotify} & \multicolumn{2}{l}{Netflix TV} & \multicolumn{2}{l}{Netflix Film} \\
Country & Best distribution & Loglikelihood & Best distribution & Loglikelihood & Best distribution & Loglikelihood & Best distribution & Loglikelihood \\
BR & Stretched exponential & -63804.4605 & Truncated powerlaw & -13952.09005 & Lognormal & -976.039065 & Lognormal & -1506.108731 \\
CA & Stretched exponential & -65111.9192 & Truncated powerlaw &  -16828.35456 & Lognormal & -1172.655954 & Lognormal & -1486.512458 \\
DE & Stretched exponential & -73416.7651 & Truncated powerlaw & -23780.34875 & Lognormal & -1070.506085 & Lognormal & -1377.749469 \\
FR & Stretched exponential & -69299.9081 & Stretched exponential & -19838.7659 & Lognormal & -1090.581559 & Lognormal &  -1444.846198 \\
GB & Stretched exponential & -64322.7649 & Truncated powerlaw & -16224.22214 & Lognormal & -1145.872704 & Lognormal & -1457.604517 \\
IN & Stretched exponential & -101575.8795 & Stretched exponential & -9858.387787 & Lognormal & -857.638549 & Lognormal & -1251.912196 \\
JP & Stretched exponential & -52606.47729 & Stretched exponential & -9806.484219 & Lognormal & -760.124471 & Lognormal &  -1386.816946 \\
KR & Stretched exponential & -54897.40738 & Truncated powerlaw & -13807.96261 & Lognormal & -697.067017 & Lognormal & -1325.809642 \\
MX & Stretched exponential & -55512.12941 & Truncated powerlaw & -10346.51229 & Lognormal & -967.651525 & Lognormal & -1516.861636 \\
US & Lognormal & -67029.40114 & Truncated powerlaw & -18026.60447 & Lognormal &  -1093.631038& Lognormal & -1394.563084
\end{tabular}
\end{table}
